Social EgoMesh Estimation

Accurately estimating the 3D pose of the camera wearer in egocentric video sequences is crucial to modeling human behavior in virtual and augmented reality applications. The task presents unique challenges due to the limited visibility of the user's body caused by the front-facing camera mounted on their head. Recent research has explored the utilization of the scene and ego-motion, but it has overlooked humans' interactive nature. We propose a novel framework for Social Egocentric Estimation of body MEshes (SEE-ME). Our approach is the first to estimate the wearer's mesh using only a latent probabilistic diffusion model, which we condition on the scene and, for the first time, on the social wearer-interactee interactions. Our in-depth study sheds light on when social interaction matters most for ego-mesh estimation; it quantifies the impact of interpersonal distance and gaze direction. Overall, SEE-ME surpasses the current best technique, reducing the pose estimation error (MPJPE) by 53%. The code is available at https://github.com/L-Scofano/SEEME.

==> sec/5_discussion.tex <==
\section{Discussion}

\TD{
\begin{itemize}
    \item Use the wearer's pose to refine EgoHMR's results.
    \item Draw a Pictorial for the model
    \item Show small variability of our model 
    \item Show ablation on different sampling numbers
\end{itemize}
}






==> sec/tables/ablation_tables.tex <==

\begin{table*}[h!t]
    \centering
    
    \resizebox{1\textwidth}{!}{
    
    \begin{tabular}{cc}
         \resizebox{.4\textwidth}{!}{
        \begin{tabular}{l|cccc}
\cline{1-5}
\multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Wearer-Interactee\\ Distance Threshold ($m$) \end{tabular}} & MPJPE ($mm$) & \begin{tabular}[c]{@{}c@{}}Orientation\\ Error\end{tabular} & \begin{tabular}[c]{@{}c@{}}Translation\\ Error ($mm$)\end{tabular} & \begin{tabular}[c]{@{}c@{}}Acceleration\\ Error ($mm/s^2$)\end{tabular} \\ 
\hline
\multicolumn{1}{c|}{-} & 126 & \textbf{0.48} & 164 & 2.67 \\
\hline
\multicolumn{1}{c|}{$d > 2$} & 132 & \textbf{0.48} & 183 & 2.76 \\ 
\multicolumn{1}{c|}{$1 < d < 2$} & 128 & 0.49 & 161 & 2.73 \\ 
\multicolumn{1}{c|}{$d < 1$} & \textbf{119} & \textbf{0.48} & \textbf{156} & \textbf{2.06} \\ 
\hline
\end{tabular}}
         &  
         \resizebox{.4\textwidth}{!}{
         \begin{tabular}{l|c|cccc}
\cline{1-6}
\multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Wearer-Interactee\\ looking at each other\end{tabular}} & FOV & MPJPE & \begin{tabular}[c]{@{}c@{}}Orientation \\ Error\end{tabular} & \begin{tabular}[c]{@{}c@{}}Translation\\ Error\end{tabular} & \begin{tabular}[c]{@{}c@{}}Acceleration\\ Error\end{tabular} \\
\hline
\multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & 126 & 0.48 & 164 & 2.67 \\
\hline
\multicolumn{1}{c|}{No} & & 127 & 0.48 & 173 & 2.71 \\
\multicolumn{1}{c|}{Yes} & \multicolumn{1}{c|}{\multirow{-2}{*}{60}} & \textbf{123} & \textbf{0.48} & \textbf{157} & \textbf{2.57} \\ 
\hline
\multicolumn{1}{c|}{No} & & 127 & 0.50 & 175 & 2.79 \\
\multicolumn{1}{c|}{Yes} & \multicolumn{1}{c|}{\multirow{-2}{*}{30}} & \textbf{117}   & \textbf{0.43} & \textbf{137} & \textbf{2.54} \\ 
\hline
\end{tabular}}
         \\
         \small{(a)} & \small{(b)} 
         
    \end{tabular}}

    \caption{
    \textit{(Left)} Ablation study on the interpersonal distance between wearer and interactee. 
    %Conditioning on the interactee's pose works best when in close proximity. 
    \textit{(Right)} Ablation study on gaze directions. 
    %By considering an angle of 60 and 30 degrees, we asses if the wearer and the interactee are looking at each other. If this is the case, the conditioning boots improve the performance even more.
    }
    \label{tab:ablation_x}
    \vspace{-.3cm}
\end{table*}



==> sec/tables/egopose_estimation_cap.tex <==
% % Please add the following required packages to your document preamble:
% % \usepackage{multirow}
% \begin{table}[!ht]
% \centering
% \resizebox{0.47\textwidth}{!}{
% \begin{tabular}{l|cc|cccc|}
% \cline{2-7}
%  & \multicolumn{2}{c|}{Conditioning} & \multirow{2}{*}{MPJPE} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Orientation \\ Error\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Translation\\ Error\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Acceleration \\ Error\end{tabular}} \\ %\cline{2-3}
% & Scene         & Interactee        &                        &                                                                               &                                                                              &                                                                                \\ \hline
% \multicolumn{1}{|l|}{EgoEgo~\cite{Zhang2021EgoBodyHB}} & \times           & \times               & 316                    & 1.56                                                                          & 315                                                                         & 5.8                                                                           \\ \hline
% \multicolumn{1}{|l|}{Ours}   & \ding{51}         &        \times      & 161                    & 0.75                                                                          & 208                                                                          & \textbf{3.57}                                                                  \\
% \multicolumn{1}{|l|}{Ours}   & \ding{51}         & \ding{51}             & \textbf{155}           & \textbf{0.73}                                                                 & \textbf{261}                                                                 & 3.34                                                                           \\ \hline
% \end{tabular}}
% \caption{Results with thresholding on capped Dataset (less frames given by SLAM).}
% \label{tab:egopose}
% \end{table}

==> sec/tables/head_estimation.tex <==
\begin{table}[h!]
\centering
\resizebox{0.47\textwidth}{!}{
\begin{tabular}{l|l|cc} \cline{1-4}
\textbf{Model}           & \textbf{Dataset Portion} & \textbf{Head Orientation Error} & \textbf{Head Translation Error} \\ \hline

{EgoEgo~\cite{Li2022EgoBodyPE}}  & Full Dataset             & 0,96                            & 632                             \\
Ours                     & Full Dataset             & 1,36                            & 489   \\ \hline


\end{tabular}}
\caption{Head Estimation Error 
}
\label{tab:head_estimation}
\end{table}

==> sec/tables/pose_estimation.tex <==
\begin{table}[!ht]
\centering
\resizebox{0.47\textwidth}{!}{
\begin{tabular}{l|ccc|cccc|}
\cline{2-8}
                                        & \multicolumn{3}{c|}{Conditioning} & \multirow{2}{*}{G-MPJPE} & \multirow{2}{*}{MPJPE} & \multirow{2}{*}{PA-MPJPE} & \multirow{2}{*}{V2V} \\
                                        & Image    & Scene   & Interactee   &                          &                        &                           &                      \\ \hline
\multicolumn{1}{|l|}{ProHMR~\cite{Kolotouros2021ProbabilisticMF}}            & \ding{51}    &         &              & 181.33                   & 72.92                  & 46.57                     & 90.88                \\
\multicolumn{1}{|l|}{ProHMR-scene-\textit{orig}} & \ding{51}    & \ding{51}   &              & 133.72                   & 73.13                  & 48.87                     & 91.59                \\
\multicolumn{1}{|l|}{EgoHMR~\cite{Liu2023EgoHMREH}}            & \ding{51}    & \ding{51}   &              & 128.62                   & 65.70                  & 47.17                     & 82.93                \\ \hline
\multicolumn{1}{|l|}{EgoHMR w/ wearer}              & \ding{51}    & \ding{51}   & GT           &   CE                      &             LA           &                FAR           &         EMO             \\
\multicolumn{1}{|l|}{EgoHMR w/ wearer}              & \ding{51}    & \ding{51}   & PRED         &                          &              DA          &           JE!                &                      \\ \hline
\end{tabular}}
\caption{Caption.}
\label{tab:poseet}
\end{table}

==> sec/tables/s1_reconstruction.tex <==
\begin{table}[]
\begin{tabular}{ccc}
\hline
\textbf{Reconstruction}                & \textbf{MPJPE}           & \textbf{RE}               \\ \hline
\textit{G.O. - Pred}                   & 114.7                    & 196.2                     \\
\multicolumn{1}{l}{\textit{G.O. - GT}} & \multicolumn{1}{l}{58.3} & \multicolumn{1}{l}{196.2} \\ \hline
\end{tabular}
\caption{Test}
\label{tab:s1_reconstruction}
\end{table}
